Revisiting the Examination Hypothesis with Query Specific Position Bias

Click through rates (CTR) offer useful user feedback that can be used to infer the relevance of search results for queries. However it is not very meaningful to look at the raw click through rate of a search result because the likelihood of a result being clicked depends not only on its relevance but also the position in which it is displayed. One model of the browsing behavior, the {\em Examination Hypothesis} \cite{RDR07,Craswell08,DP08}, states that each position has a certain probability of being examined and is then clicked based on the relevance of the search snippets. This is based on eye tracking studies \cite{Claypool01, GJG04} which suggest that users are less likely to view results in lower positions. Such a position dependent variation in the probability of examining a document is referred to as {\em position bias}. Our main observation in this study is that the position bias tends to differ with the kind of information the user is looking for. This makes the position bias {\em query specific}. In this study, we present a model for analyzing a query specific position bias from the click data and use these biases to derive position independent relevance values of search results. Our model is based on the assumption that for a given query, the positional click through rate of a document is proportional to the product of its relevance and a {\em query specific} position bias. We compare our model with the vanilla examination hypothesis model (EH) on a set of queries obtained from search logs of a commercial search engine. We also compare it with the User Browsing Model (UBM) \cite{DP08} which extends the cascade model of Craswell et al\cite{Craswell08} by incorporating multiple clicks in a query session. We show that the our model, although much simpler to implement, consistently outperforms both EH and UBM on well-used measures such as relative error and cross entropy.

==> abstract.tex <==
Eliminating Position Bias From Click Data

Click logs contain useful user feedback that can be used to infer the
relevance of search results for queries.  For instance you can look at
click through rate, which is the fraction of impressions that resulted
in clicks for a given url, to measure the relevance feedback of a
document for a given query.  However, users typically assume better
documents to be placed higher resulting impressions at higher
positions having a higher click through rate than those at lower
positions.  Such a variation in click through rate, specifically due
to the position of the impression, is referred to as {\em position
bias}.  A simple analysis of aggregating the click through rates over
all queries shows a decreasing value of the position bias from higher
to lower positions except for a small increase at the last position on
the result page.

However, analyzing the position bias curve aggregated over all queries
is not sufficient since the position bias tends to be different for
different queries.  For example, a navigational query such as {\tt
cnn} tend to have a different bias curve from an informational queries
{\tt alzheimers disease}.  In this study, we present a model for
analyzing a query specific position bias from the click data and use
these biases to derive position independent relevance of search
results. For a given query, the position bias is assumed to be
independent of the document. Our model is based on the assumption that
for a given query, the click through rate $CTR(d,j)$ of a document $d$
at position $j$ is proportional to the product of its relevance $R_d$
and position bias $c_j$.  Based on this model and its variants, we
learn the parameters $R_d$ and $c_j$ for different queries.  We
evaluate the performance of our learnt relevance measure and compare
it to other ranking features like {\em bm25f} and {\em page rank}
using NDCG, MAP, and MRR scores.

